Building a Village: A Multi-stakeholder Approach to Open Innovation and Shared Governance to Promote Youth Online Safety

The SIGCHI and Social Computing research communities have been at the forefront of online safety efforts for youth, ranging from understanding the serious risks youth face online to developing evidence-based interventions for risk protection. Yet, to bring these efforts to bear, we must partner with practitioners, such as industry stakeholders who know how to bring such technologies to market, and youth service providers who work directly with youth. Therefore, we interviewed 33 stakeholders in the space of youth online safety, including industry professionals (n=12), youth service providers (n=11), and researchers (n=10) to understand where their visions toward working together to protect youth online converged and surfaced tensions, as well as how we might reconcile conflicting viewpoints to move forward as one community with synergistic expertise on how to change the current sociotechnical landscape for youth online safety. Overall, we found that non-partisan leadership is necessary to chart actionable, equitable goals to facilitate collaboration between stakeholders, combat feelings of isolation, and foster trust between the stakeholder groups. Based on these findings, we recommend the use of open-innovation methods with their inherent transparency, federated governance models, and clear but inclusive leadership structures to promote collaboration between youth online safety stakeholders. We propose the creation of an open-innovation organization that unifies the diverse voices in youth online safety to develop open-standards and evidence-based design patterns that centralize otherwise fragmented efforts that have fallen short of the goal of effective technological solutions that keep youth safe online.

==> 04-results-rq1-table.tex <==
\begin{table}[htp]\small
\caption{Stakeholder preference for non-partisan leadership through common goals (RQ1)}
\label{tab:codebook_rq1-study3}
\centering

\begin{tabular}{>{\raggedright}p{0.2\textwidth}>{\raggedright}p{0.27\textwidth}p{0.4\textwidth}}
\toprule
\textbf{Theme}                                                      & \textbf{Sub-Themes} & \textbf{Quote} \\ \midrule

\multirow{2}{=}{Youth online safety is a big problem that needs innovative solutions} 
& \textit{Won't fix itself (General Importance)} &  \textit{``It's a huge problem, but it's not a huge problem that's going to fix itself within this, within the problem. It's going to have to be attached to the problem, but it can't replicate the problem.''} - P30, Service Provider (Educator) \\\cline{2-3}
& \textit{Individual platforms have a conflict of interest} &  \textit{``I don't know right now, as I'm sitting here thinking raw, I'm thinking third party might be the way to go because you're not beholden to the platform, the social media platform. You're not owned by them. It, it's kinda like conflict of interest.''} - P26, Service Provider (Educator)\\ \cline{1-3}

\multirow{2}{=}{Non-partisan leadership is necessary for creating effective solutions} 
& \textit{Individuals don't have the time to contribute without third-party oversight facilitating collaborative efforts} &  \textit{``
I would certainly be open to, you know being a research partner and, and and signing on to research projects that I think are interesting. But it wouldn't, I, I just don't see myself browsing you know, browsing projects to say, Hmm! Where can I fit in?''} - P23, Service Provider (Case Manager) \\\cline{2-3}
& \textit{Someone has to be accountable for quality} &  \textit{``...you know, the reason why people like nuance from Microsoft so much versus some of the other possible competitors that are open source and held a lot cheaper is I can sue Microsoft. Right. If there's a problem, I can sue them.''} - P28, Industry  (Entrepreneur)\\ \cline{1-3}

\multirow{2}{=}{We need a common goal that does not try to boil the ocean} 
& \textit{Non-proprietary collaboration on outcomes needed to promote community} &  \textit{``I think that would need some careful thought, because I would be kind of pissed off if I mean, you know, like what I just put up there. I am definitely not the only one who's thinking about this, so I guess whatever I would propose would be general enough like I wouldn't give away if I had a particularly interesting angle that I wanted to keep to myself''} - P15, Researcher \\\cline{2-3}
& \textit{Need integrated solutions that are not platform dependent} &  \textit{``What I don't want is to become connected with like, I don't need another network. I like, I'm on Twitter. I'm on Linkedin. I'm like, I have all those connections. I don't want to have to re-engage all those connections.''} - P30, Service Provider (Educator)
\\\bottomrule
\end{tabular}
\end{table}
%\FloatBarrier

==> 04-results-rq1.tex <==
\subsection{We Will Help, If Someone Takes Charge (RQ1)} %\ref{tab:codebook_rq1-study3}
RQ1 examined the areas where secondary stakeholders in youth online safety agree in the context of developing technology-driven online safety solutions for youth. Their views were grouped under three major themes: 1) innovative solutions are needed, 2) non-partisan leadership is necessary, and 3) common goals need to be defined. These themes are shown in \hyperref[tab:codebook_rq1-study3]{Table \ref{tab:codebook_rq1-study3}}. We now present these themes.

\subsubsection{Innovative Solutions Needed}
Under the theme of needing innovative solutions, participant responses were further grouped under two sub-themes: 1) the problem of youth online safety is important and won't fix itself, and 2) someone other than youth-facing internet companies should lead the efforts as those companies have a conflict of interest. We expand on these below.

\input{04-results-rq1-table}

\paragraph{The problem won't fix itself:} All participants viewed youth online safety as an important topic and perceived efforts in this stream to be worthy of commendation. Participants thought the design of youth safety technology being informed by inputs from broader society was important even if they thought \textit{more} technology wasn't the answer to the issues faced by youth and adults. Sentiments ranged from the need to celebrate every small success in youth protection, to feelings of being thankful for efforts as there are never enough resources and individuals fighting for youth. The underlying idea shared by participants was that \textit{something} is needed to help improve the complex relationships that exist between youth, parents/guardians, and technology, given the perceived harm youth are exposed to online. They thought uncovering what that something is needed to be done inclusively because of the prevalence of youth internet usage and varying views of the public.
\xquote{I don't think that there's a person walking the street that does not have an opinion about device driven life now.}{P26, Service provider (Educator)}
Regardless of the primary interest of any stakeholder group, they viewed the other groups as necessary in the creation and promotion of safety efforts to enhance end-user trust. In this regard, service providers placed importance on stakeholders who have direct day-to-day access to youth as they have the capability of finding out what youth are doing sooner. Contrastingly, the same group also lamented that they tend not to know solutions to online issues faced by youth especially due to the fast rate of change of online technologies. Participants acknowledge that parents and youth seek help from online sources but stated that this has both positive and negative implications. While it was good that the individuals sought help, the issues of information overload and extreme or incorrect information being shared with no contextual filter were seen as harmful.
\xquote{The Internet is a fire hose of information. Some of it is not good or shows extremes that aren't really reality or whatever up. So I think from a parent perspective it's a lot of concerns along those lines. And then that bleeds into a lot of times, I'm sure, and what I see is in school administration counselors, etc, trying to explain stuff to the parents who don't really understand, understand their concerns.}{P26, Service provider (Educator)}
To combat these harms, each stakeholder group expressed interest in the concepts behind the design probe tools used in the study in line with their stakeholder role. This interest, which will be discussed further in RQ2, was expressed in how best they could extract value from the probes to fulfill their roles. They all, however, stated that youth-facing internet companies should also be part of the discussion, but had reservations about them doing so, leading to the next sub-theme. 

\paragraph{Individual Platforms have Conflicting interests:} Participants viewed social media companies as needing to do a better job regarding youth online protective measures, or the perceived lack thereof. In discussing this, participants viewed social media companies' goal of consistent user engagement for profit versus the protections they are asked to implement as a conflict and expressed distrust in the motivations of those companies to implement those measures transparently. Service providers raised this as a concern especially when dealing with youth who have are victims of crimes.
\xquote{We get some of our referrals from law enforcement if obviously an Internet crime against a child has been committed and I think they have a lot of trouble of getting information from Snapchat, even when a child has been victimized or solicited by an adult.}{P6, Service Provider (Case Worker)}
Given the context of conflicting interests being present, the idea of a third party taking the lead to promote youth online safety was seen as favorable. Participants viewed establishing such a third party as engendering more trust from the public by not having the stigma associated with social platforms. There was a preference for such an effort to be undertaken by, or attached to, an already well-known, publicly trusted organization to avoid unnecessary effort to get a new community going, the cold-start problem\footnote{The cold-start problem is the name given to the situation where a new item or product takes a long time to make an impact due to being unknown by its target population.}, and also to avoid the public possibly distrusting new or small organizations given the high-stakes in the context of youth online safety.
\xquote{My immediate thought is you would want it to be a standalone because you don't want the baggage that comes with the others.}{P24, Service provider (Educator)}



\subsubsection{Non-partisan leadership is necessary for creating effective solutions}
\par The theme of non-partisan leadership for creating effective solutions groups two sub-themes: 1) individuals having limited time to contribute to community-led youth protection efforts, and 2) holding someone accountable. These sub-themes emerged from participants reflecting on how they and stakeholders in similar roles would collaborate on youth protection efforts. We expand on these below.

\paragraph{Individuals have no time to contribute:}Participants expressed apprehension about randomly reaching out to others, even if they knew they were working in the same field. Instead, they preferred reaching out to, and being reached out to, when there was some commonality between the parties involved. As such, they discussed the community being grown \textit{organically}, that is, through working on common goals. They did not see themselves, or others, actively searching for projects in the space of youth online safety to work on. In discussing this, they noted feeling isolated in their efforts to protect youth as they execute the duties of their stakeholder role. Youth online safety communities providing opportunities to network \textit{based on common, narrowly defined goals} was seen as the path forward to gain adoption and engagement. These opportunities were not only on the online modality but also in-person, as participants viewed the online community as the place where the work is documented, but offline being where the community truly exists.
\xquote{I think, like, so there has to be a really good way, to sort of differentiate between the types of projects and cause. If not like, I just feel like it's gonna be a dump of projects and like nobody's gonna sift through them.}{P21, Researcher}
In doing this, the expectation was that community leadership would define the goal(s) the community works on. This was seen as providing clear community goals leading to accountability, clear messaging on membership fit, and expected contribution levels. While participants suggested that the community should work, and build membership on a common goal, they noted that they and others are busy and thus guard access to their time. Expecting them to submit new project proposal ideas or heavily contribute to projects was therefore questionable. However, they also expressed a sense of responsibility and altruism in that they were willing to find the time to put towards the cause if their assignments could be explicitly stated, and if they were asked directly to fill a need. From a community-wide perspective, participants expect the community software implementation to cater to this by allowing them to contribute their knowledge asynchronously through knowledge bases and question+answer formats. This would allow members to passively contribute to the community while not placing strict demands on their already constrained time.
\xquote{I, personally would love you know, a world leading community that summarized the peer reviewed research and had that in ways that was very accessible... if someone can summarize it and and put it in a digestible form for young people or for parents... That kind of, you know, shows the benefits and shows the drawbacks, and so on, would be helpful.}{P29, Industry (Entrepreneur)}

%\paragraph{Someone Has to Hold Accountability:} In wanting to be credited for their work, and credit others (which will be addressed in RQ2), participants expressed the need for individuals to hold someone accountable in less than favorable conditions. This was expressed in two ways. Firstly, participants viewed open innovation initiatives with skepticism regarding the longevity and availability of ongoing maintenance of the projects. Skepticism also was shown toward the perceived lack of being able to hold the open innovation project accountable for poor performance. Secondly, participants mostly in the service provider group, expressed the need for a resource to turn to when they need the resource that has the answers to their issues. The participants expressed a need to hold someone accountable to have the knowledge they don't and to keep abreast with the challenges youth face. This knowledge was seen as being the value of community participation.
%\xquote{The lead feature should not be, hey, we're going to get together and solve problems online. The problem to me is, I don't know what the problems are right. And so like, there's this things I know, and things I don't know... But the things I don't know about are things that I think you know [the community] could help with... and that's where the community can come in.}{P30, Service Provider (Educator)}

\subsubsection{Work on a common goal. Don't boil the ocean} The final major theme in RQ1 captures stakeholder overarching views on how the community should work on selected outcomes. Two sub-themes emerged when they considered this: 1) collaboration on non-proprietary outcomes being needed to promote community, and 2) the need for integrated solutions.

\paragraph{Non-proprietary collaboration needed to promote community:} When considering the possible outputs from the community, and working on those outputs, participants thought an open innovation approach would be nice but cautioned about its use in the US. Participants viewed open innovation and open-source methodologies as being more successful in Asia and Europe due to the existing legal framework and perceived open-source friendly developer environment in those regions. Participants in the industry and research groups were mostly concerned about protecting proprietary information. Researchers were concerned about having their research ideas stolen and implemented without credit being given as their research is intricately linked to academic tenures. Industry participants shared that during community participation they probably would intentionally, sometimes due to legal repercussions for failure, not share information about upcoming products or features (trade secrets) since competitors might also be present in communities. Service providers thought that community administration would not need to worry about proprietary protections as information shared by members would be self-selecting, that is, members would naturally choose not to overshare when necessary.
\xquote{Let's start with the fact that this is a naturally very competitive space... There's the perspective that engaging in an open source project means giving away one's intellectual property and therefore losing rights to commercialize or monetize their work... A lot more progress could be made if organizations and founders were willing to work together. But yeah, capitalism gets in the way of that.}{P14, Researcher}

\paragraph{Integrated \& Platform-Independent Solutions are Needed:} Participants expressed a need for integrated solutions by showing a disdain for installing more applications on their devices and also expressing displeasure at the prospect of visiting or interacting with another online platform. These pain-points were shared from the perspectives of interacting with youth online communities in the role of a product creator or external consultant through online modalities, and also from the perspective of parents/guardians not wanting a youth protection tool disjointed from social media offerings.
\xquote{Okay, so right off the bat, it's yet another community to join and another site to log into and my, my first question would be you, you might be better served  by presenting [the community] starting with something like Facebook, which already has really robust community-based tools versus starting to build your own.}{P25, Industry (Tech Consultant)}
This sentiment prevailed as participants considered what communities of this nature would need to provide to potential members to engage them on such platforms. Suggestions tended to be features commonly found on social media platforms such as making provisions for liking/disliking posts and user interfaces styled after contemporary social or professional platforms. While there was a preference for having a standalone platform which \textit{does not repeat the same mistakes} as social media platforms, a new platform rehashing features commonly associated with current social media platforms to encourage engagement carries the possibility of participants being overwhelmed as exemplified in the following quote:
\xquote{I hate and love Slack. Like I use it every day, but like, I have so many. I only really, I, they're just too many channels that I'm part of. And so that would quickly, I would probably not go to that anymore.}{P25, Industry (Tech Consultant)}
The need for integration was further reinforced by participants stating that they generally now spend little time using social platforms even if they were previously avid users. They spoke of intentionally deactivating accounts on social platforms for various reasons such as time constraints, data use concerns, and differing views with platform leadership. In summary, participants saw the need to avoid application fatigue by having the community seek them out instead of reverse.


